Human Centered AI for Indian Legal Text Analytics

Legal research is a crucial task in the practice of law. It requires intense human effort and intellectual prudence to research a legal case and prepare arguments. Recent boom in generative AI has not translated to proportionate rise in impactful legal applications, because of low trustworthiness and and the scarcity of specialized datasets for training Large Language Models (LLMs). This position paper explores the potential of LLMs within Legal Text Analytics (LTA), highlighting specific areas where the integration of human expertise can significantly enhance their performance to match that of experts. We introduce a novel dataset and describe a human centered, compound AI system that principally incorporates human inputs for performing LTA tasks with LLMs.

==> extra.tex <==

\begin{lstlisting}[caption={Sample LLaMA-2 Prompt}]
[INST]Given below are four pairs of legal documents. You have been presented with some parts of these documents and whether they are similar or not. Try to answer for Document 9 and Document 10.

### Document 1: 22\. In the light of the foregoing discussion, we allow the appeals, set aside the impugned ...
### Document 2: the suit or application the Court should accept that the statements made in the plaint/application are ...
### Similarity: Yes

### Document 3: filed, unacceptable. Learned counsel for the respondent submitted that the Court could not have granted ...
### Document 4: right. By adopting the latter course indicated by us, the defendants first set would have got a fair ...
### Similarity: No

### Document 5: iv) ""Hits of Salman Khan"" v) ""Hum Aapke Hai Kaun"". However, I may clarify that it shall be open to ...
### Document 6: flights can not be a ground to prevent the passengers on board from returning to the airport lounge ...
### Similarity: No

### Document 7: An advocate abusing the process of court is guilty of misconduct. When witnesses are present in the ...
### Document 8: complying with the legal provisions contained in Section 309 of the Code. Of course, the High Court ...
### Similarity: Yes

### Document 9: the order passed by the learned Trial Judge we wish to make it clear that our aforesaid conclusion ...
### Document 10: ... Even in the light of the principles highlighted above when the evidence is tested, the inevitable ...    
### Similarity: ?

Similarly, are the given parts of Legal Document 9 and Legal Document 10 similar apart from the fact that they contain discussions of legal terms? Give a one word response: Yes or No.[/INST] 
\end{lstlisting}


\begin{lstlisting}
These are the few examples of questions pertaining to the Indian Constitution, judiciary, legislative, and various socio-political issues in India. 
<Examples>

Context:The 'Doctrine of Basic Structure' was propounded by the Indian Supreme Court to limit the amendment power of the Parliament. It holds ...
Question: Can you interpret the implications of the 'Doctrine of Basic Structure' in the Indian Constitution?

Context:To: The Hon'ble District and Sessions Judge, [Location]. Subject: Application for Anticipatory Bail under Section ...
Question: How would you draft an anticipatory bail application under Section 438 of the Code of Criminal Procedure, 1973?

Context:Honourable court, my client has been unjustly accused of defamation. However, as the evidence will show, my ...
Question: Can you write an opening statement for a defense attorney in a defamation case under Indian law?

Context:In Vishaka v. State of Rajasthan, the Supreme Court recognized sexual harassment at the workplace as a ...
Question: Can you provide a brief analysis of the legal case: 'In Vishaka v. State of Rajasthan, the Supreme Court of India gave guidelines on sexual harassment at the workplace.'?

Context:The principle of 'audi alteram partem', or 'hear the other side', is a fundamental principle of natural ...
Question: How relevant is the principle of 'audi alteram partem' in administrative law?

Context:A 'National Climate Court', if established in India, could ...
Question: Explain the idea of a 'National Climate Court' and its potential role in India?

Context:The Indian Evidence Act, 1872 provides the rules for what evidence is admissible in court. It ...
Question: Can you summarize the main tenets of the Indian Evidence Act, 1872?

Context:'Double Jeopardy' is a constitutional safeguard under Article 20(2) which prohibits a person from ...
Question: Can you explain the concept of 'Double Jeopardy' under Article 20(2) of the Indian Constitution with a relevant case law?

Context:The petitioner's argument in this case expanded the scope of personal liberty under Article 21. While  ...
Question: How would you critique the legal arguments presented in the case of Maneka Gandhi v. Union of India?

Context:The Ayodhya Verdict settled a long-standing dispute over a religious site in Ayodhya. The Supreme ...
Question: Can you analyze the legal implications of the Ayodhya Verdict by the Supreme Court of India?

</Examples>
<Provided context>

At the outset, it was noticed that arguments on this application were partly heard by the predecessor Bench on 19.10.2022. The Court was therefore inclined to place the application for ...

</Provided context>
The output should be formatted as a JSON instance that conforms to the JSON schema ...

Walk me through this provided context in manageable parts, step by step, summarizing and analysing as we go and generate the multiple questions from the given context. The generated questions should be similar to question as in examples. The only thing generated should be the questions and corresponding sub-context (from provided context) from which the question is generated.'

\end{lstlisting}

\begin{lstlisting}
CREATE TABLE Cases (
    CaseID INT PRIMARY KEY,
    CaseName VARCHAR(255),
    CourtName VARCHAR(255),
    DateFiled DATE
);
CREATE TABLE Plaintiffs (
    PlaintiffID INT PRIMARY KEY,
    CaseID INT,
    PlaintiffName VARCHAR(255),
    PlaintiffNumber VARCHAR(255),
    FOREIGN KEY (CaseID) REFERENCES Cases(CaseID)
);
CREATE TABLE Trademarks (
    TrademarkID INT PRIMARY KEY,
    PlaintiffID INT,
    TrademarkName VARCHAR(255),
    TrademarkNumber VARCHAR(255),
    Class INT,
    ProductCategory VARCHAR(255),
    FOREIGN KEY (PlaintiffID) REFERENCES Plaintiffs(PlaintiffID)
);
CREATE TABLE Copyrights (
    CopyrightID INT PRIMARY KEY,
    PlaintiffID INT,
    CopyrightName VARCHAR(255),
    RegistrationNumber VARCHAR(255),
    Class INT,
    ProductCategory VARCHAR(255),
    FOREIGN KEY (PlaintiffID) REFERENCES Plaintiffs(PlaintiffID)
);
CREATE TABLE Injunctions (
    InjunctionID INT PRIMARY KEY,
    CaseID INT,
    InjunctionType VARCHAR(255),
    OrderDate DATE,
    FOREIGN KEY (CaseID) REFERENCES Cases(CaseID)
);
CREATE TABLE SettlementAgreements (
    AgreementID INT PRIMARY KEY,
    CaseID INT,
    AgreementDate DATE,
    TermsAndConditions TEXT,
    FOREIGN KEY (CaseID) REFERENCES Cases(CaseID)
);
CREATE TABLE AgreementClauses (
    ClauseID INT PRIMARY KEY,
    AgreementID INT,
    ClauseNumber VARCHAR(255),
    ClauseSummary TEXT,
    FOREIGN KEY (AgreementID) REFERENCES SettlementAgreements(AgreementID)
);
\end{lstlisting}
